Resetting the Optimizer in Deep RL: An Empirical Study

We focus on the task of approximating the optimal value function in deep reinforcement learning. This iterative process is comprised of solving a sequence of optimization problems where the loss function changes per iteration. The common approach to solving this sequence of problems is to employ modern variants of the stochastic gradient descent algorithm such as Adam. These optimizers maintain their own internal parameters such as estimates of the first-order and the second-order moments of the gradient, and update them over time. Therefore, information obtained in previous iterations is used to solve the optimization problem in the current iteration. We demonstrate that this can contaminate the moment estimates because the optimization landscape can change arbitrarily from one iteration to the next one. To hedge against this negative effect, a simple idea is to reset the internal parameters of the optimizer when starting a new iteration. We empirically investigate this resetting idea by employing various optimizers in conjunction with the Rainbow algorithm. We demonstrate that this simple modification significantly improves the performance of deep RL on the Atari benchmark.

==> Background.tex <==
\section{Background}
In this section, we establish our notation, and present a background on reinforcement learning and optimization.

\subsection{Reinforcement Learning}
Reinforcement learning (RL) is the study of artificial agents that use their environmental experience to find behavior that maximizes an evaluative feedback in the form of a reward signal~\citep{littman_evaluative, rl_book}. The Markov Decision Process~\citep{PutermanMDP1994}, or MDP in short, is used to mathematically define the RL problem. An MDP is specified by a tuple $\langle \mathcal{S,A,R,P,\gamma}\rangle$, where $\mathcal{S}$ is the set of states and $\mathcal{A}$ is the set of actions. The functions $\mathcal{R:S\times A\rightarrow}\ \mathbb R$ and $\mathcal{P:S\times A \times S\rightarrow}\ [0,1]$ denote the reward and state transition probabilities of the MDP, respectively. Finally the scalar $\gamma$ discounts rewards that are received in the future.

A fundamental goal in RL is to learn a policy, a mapping from states to a probability distribution over actions, ${\pi:\mathcal{S}\rightarrow \mathcal{P}(\mathcal{A})}$, that obtains high sums of future discounted rewards. An important object in RL is the state value function. Formally, it denotes the expected discounted sum of future rewards when committing to a policy $\pi$ in a state $s$, and is defined by $v^{\pi}(s)\myeq \E\big[\sum_{t=0}^{\infty}\gamma^{t} R_t\big |S_0=s, \pi \big]$. Another important object in RL is the Bellman operator $\mathcal{T^{\pi}}$, which is associated with the mapping $\pi$, and is defined by
\begin{equation*} \label{eq:Bellman}
\big[\mathcal{T^{\pi}}v\big](s):=\!\sum_{a\in\mathcal{A}}\pi(a\mid s)\big(\mathcal{R}(s,a)+\gamma\!\sum_{s'\in \mathcal{S}}\! \mathcal{P}(s,a,s') v(s')\big).
\end{equation*}

==> tasks.tex <==
\section{Tasks}
\begin{itemize}
    \item {\bf Writing the proof for the non-prox setting}.
    \item {\bf Investigating the linear case with the squared loss as a special case of the theory}.
    \item Discussing the simple examples (2 examples from the book).  \\ http://www.incompleteideas.net/book/RLbook2020.pdf (section 11)
    \item what is known about convergence of TD? Kavosh: TD with linear function approximation and on-policy updates, we get convergence. Remove on-policy or lineraity and we will diverge.
    see this paper: 
    \href{https://www.mit.edu/~jnt/Papers/J063-97-bvr-td.pdf}{paper}
    \href{https://proceedings.neurips.cc/paper_files/paper/1996/file/e00406144c1e7e35240afed70f34166a-Paper.pdf}{paper}
    and this one \href{https://arxiv.org/abs/1904.10945}{paper}
    logistic Q learning \href{https://arxiv.org/pdf/2010.11151v1.pdf}{paper}
    \item what is different H?
    \item Check if the prox proof work with only convexity of $h$.
    \item Lihong suggests these papers:
    \href{http://www.machinelearning.org/archive/icml2008/papers/652.pdf}{melo}
    \href{https://www.jmlr.org/papers/volume9/munos08a/munos08a.pdf}{munos and csaba}
    \href{https://www.csd.uwo.ca/~dlizotte/publications/lizotte11convergent.pdf}{dan lizotte}
    \item {\bf Can we prove that strong convexity is must for convergence (in terms of contraction) of TD?}
    \item What is TD? Is it an algorithm? Is it a class of algorithms? RL people will think about it as the exact argmin of h? People will think about it as optimization algorithm?
\end{itemize}

